Contrastive Document Representation Learning with Graph Attention Networks

Recent progress in pretrained Transformer-based language models has shown great success in learning contextual representation of text. However, due to the quadratic self-attention complexity, most of the pretrained Transformers models can only handle relatively short text. It is still a challenge when it comes to modeling very long documents. In this work, we propose to use a graph attention network on top of the available pretrained Transformers model to learn document embeddings. This graph attention network allows us to leverage the high-level semantic structure of the document. In addition, based on our graph document model, we design a simple contrastive learning strategy to pretrain our models on a large amount of unlabeled corpus. Empirically, we demonstrate the effectiveness of our approaches in document classification and document retrieval tasks.

==> tables/datasets.tex <==
\begin{table}[ht]
\centering
\scriptsize
\begin{tabular}{llll}
\toprule
Dataset       & Count (train/dev/test) & \# classes & Avg length \\
\midrule
ArXiv         & 25,568 / 3,196 / 3,197      & 11         &  10,536      \\
Hyperpartisan & 516 / 64 / 65      & 2          &  565         \\
IMDB          & 24,000 / 1,000 / 25,000 & 2          &  231          \\
NewsGroup   & 10,182 / 1,132 / 7,532  & 20         &  314         \\
\bottomrule
\end{tabular}
\caption{Statistics of document classification datasets.}
\label{tab: dc_datasets}
\end{table}

==> tables/doc_classification_linear.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{llcccc}
\toprule
\textbf{Model} & \textbf{Finetuning} & \textbf{ArXiv} & \textbf{Newgroup} & \textbf{IMDB} & \textbf{Hyperpartisan} \\
\midrule
Roberta & Linear & 75.76   & 71.60   & 89.72   & 84.62   \\
Longformer & Linear & 65.84   & 62.36   & 88.18   & 86.15   \\
BigBird & Linear & \textbf{76.73  } & 69.05   & \textbf{89.90  } & 83.08   \\
Graph-roberta & Linear & 76.54   & \textbf{75.46  } & 88.63   & \textbf{90.57  } \\
\bottomrule
\end{tabular}
\caption{Linear Classification Accuracy on different document representation models with the document encoder frozen. The numbers are in percent.}
\label{tab:dc-linear}
\end{table*}
